Incorporating Degradation Estimation in Light Field Spatial Super-Resolution

Recent advancements in light field super-resolution (SR) have yielded impressive results. In practice, however, many existing methods are limited by assuming fixed degradation models, such as bicubic downsampling, which hinders their robustness in real-world scenarios with complex degradations. To address this limitation, we present LF-DEST, an effective blind Light Field SR method that incorporates explicit Degradation Estimation to handle various degradation types. LF-DEST consists of two primary components: degradation estimation and light field restoration. The former concurrently estimates blur kernels and noise maps from low-resolution degraded light fields, while the latter generates super-resolved light fields based on the estimated degradations. Notably, we introduce a modulated and selective fusion module that intelligently combines degradation representations with image information, allowing for effective handling of diverse degradation types. We conduct extensive experiments on benchmark datasets, demonstrating that LF-DEST achieves superior performance across a variety of degradation scenarios in light field SR.

==> includesAndMacros_yagiz.tex <==
% For author citing
%\usepackage{natbib}

% Yagiz - For the latex + Inkscape vector figure
%\usepackage{rotating}
% Yagiz - Strike through text
%\usepackage[normalem]{ulem}
% Yagiz - To scale the table
\usepackage{graphics}
%\usepackage{arydshln}
% Yagiz - Color names for text
\usepackage[usenames,dvipsnames,table]{xcolor}
%\PassOptionsToPackage{table}{xcolor}
% Yagiz - to add more spacing in tabular (table) environment
\usepackage{array}
% Yagiz - Vertical multirow cells in tables
\usepackage{multirow}
% Tunc
\usepackage{wrapfig}
\usepackage{hhline}
% Yagiz - Checkmark
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% Figure file shortcut
\newcommand{\putfigure}[1]{\input{imagetex/#1.tex}}

% Yagiz - commonly used shortcuts
\newcommand{\showimagew}[2][\linewidth]{\includegraphics[width={#1}]{{#2}}}
\newcommand{\showimageh}[2][\linewidth]{\includegraphics[height={#1}]{{#2}}}
%\newcommand{\etal}{\textit{et al.} }
%\newcommand{\etal}{et al. }
%\newcommand{\ie}{\textit{i.e.} }
%\newcommand{\eg}{\textit{e.g.} }
\DeclareMathOperator*{\argmin}{arg\,min} % argmin
\DeclareMathOperator*{\argmax}{arg\,max} % argmax
\newcommand{\ve}{\boldsymbol} % vector notation
\newcommand{\refeq}[1]{(\ref{#1})} % 
\newcommand{\reffig}[1]{Figure~\ref{#1}} % Referencing equations in the text
% For the benchmark table
\newcommand{\topscore}[1]{\textcolor{blue}{\textbf{#1}}} % vector notation
% Fixed-width centered column type
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
% Negative vspace after figures
\newcommand{\negvspace}{\vspace{-0.2cm}}
% For changes
%\newcommand{\revision}[1]{#1}%{\textcolor{red}{#1}}%}
%\newcommand{\addText}[1]{\textcolor{MidnightBlue}{#1}}
%\newcommand{\addText}[1]{#1}
%\newcommand{\deleteText}[1]{\textcolor{Maroon}{#1}}
%\newcommand{\deleteText}[1]{}

